Rating Multi-Modal Time-Series Forecasting Models (MM-TSFM) for Robustness Through a Causal Lens

AI systems are notorious for their fragility; minor input changes can potentially cause major output swings. When such systems are deployed in critical areas like finance, the consequences of their uncertain behavior could be severe. In this paper, we focus on multi-modal time-series forecasting, where imprecision due to noisy or incorrect data can lead to erroneous predictions, impacting stakeholders such as analysts, investors, and traders. Recently, it has been shown that beyond numeric data, graphical transformations can be used with advanced visual models to achieve better performance. In this context, we introduce a rating methodology to assess the robustness of Multi-Modal Time-Series Forecasting Models (MM-TSFM) through causal analysis, which helps us understand and quantify the isolated impact of various attributes on the forecasting accuracy of MM-TSFM. We apply our novel rating method on a variety of numeric and multi-modal forecasting models in a large experimental setup (six input settings of control and perturbations, ten data distributions, time series from six leading stocks in three industries over a year of data, and five time-series forecasters) to draw insights on robust forecasting models and the context of their strengths. Within the scope of our study, our main result is that multi-modal (numeric + visual) forecasting, which was found to be more accurate than numeric forecasting in previous studies, can also be more robust in diverse settings. Our work will help different stakeholders of time-series forecasting understand the models` behaviors along trust (robustness) and accuracy dimensions to select an appropriate model for forecasting using our rating method, leading to improved decision-making.

==> AIES2024/sections/background.tex <==
\section{Related Work}
We now contextualize our work with related literature so that our contributions are highlighted. We cover MM-TSFM, adversarial attacks in finance, causal analysis in time-series forecasting, and rating of AI systems. 

\subsection{Multi-modal Time-series Forecasting}

Time-series forecasting is the problem of predicting a quantity at a future time given a history of the quantity indexed with time. 
This is a well-studied problem - we review only some recent advances.

In \cite{jia2024gpt4mts}, the authors propose a prompt-based LLM framework called GPT4MTS to utilize the numerical data and articles containing information about events. \cite{jin2023time} employs a reprogramming strategy to adapt Large Language Models (LLMs) for general time series forecasting without altering the underlying language model. \cite{ekambaram2020attention} addresses the challenge of forecasting sales for newly launched products using attention-based multi-modal encoder-decoder models that use product images and other provided attributes. \cite{cheng2022financial} introduces a multi-modal graph neural network to learn from multi-modal inputs. Additionally, \cite{yu2023temporal} leveraged multi-modal data including publicly available historical stock prices, company metadata, and historical economic news in their use of LLMs for conducting explainable time series forecasting. However, in these works, the data was collected from multiple sources (numerical, news articles, etc.) to train their models. In contrast, in \cite{zeng2023from}, the authors introduce a vision transformer that uses time-frequency spectrograms as the visual representation of time-series data transforming numerical data into a multi-modal form. Their experiments demonstrate the benefit of using spectrograms augmented with numeric time series and vision transformers for learning in both time and frequency domains compared to other existing image-based and numerical approaches. We compliment their work by proposing a method to rate different MM-TSFM for robustness using a causally grounded setup. Specifically, we evaluate two variations of ViT-num-spec model introduced in \cite{zeng2023from}.


\subsection{Adversarial Attacks in Finance Domain}
Malicious agents are incentivized to attack ML models deployed by financial institutions for financial gains, especially considering that the most efficient models utilize deep-learning architectures resembling those in the NLP community, which pose a challenge due to their vast number of parameters and limited robustness.
% \cite{gallagher2022investigating} shows how the Fast Gradient Signed Method (FGSM) attack, a Single Value attack, and a label Flip attack on Convolutional Neural Network model used for time series classification, can impact the performance of the model.


\cite{nehemya2021taking} shows the vulnerability of algorithmic trading systems to adversarial attacks by demonstrating how attackers can manipulate input data streams in real-time using imperceptible perturbations, 
% ultimately deceiving trading algorithms and 
highlighting the need for mitigation strategies in the finance community.
\cite{fursov2021adversarial} studies adversarial attacks on deep-learning models on transaction records, common in finance, demonstrating vulnerabilities. 
% They also propose defenses to enhance the model robustness, thereby promoting wider adoption in banking and finance. 
\cite{xu2021adversarial} was one of the first works to consider the vulnerability of deep learning models to adversarial time series examples in which they add noise to time-series plots to attack a ResNet model. 
However, none of these works evaluate multi-modal models against such attacks, nor do they explore multi-modal attacks or perturbations. In our work, we address several perturbations most of which can be applied to uni-modal or multi-modal systems.
% that could have significant real-world impacts. Furthermore, our perturbation evaluation setup is causally grounded that helps in identifying and quantifying isolated impact of different perturbations in the presence of other attributes. 
We use both common data errors and attacks as motivations for the introduced input perturbations that we use to measure the robustness of time-forecasting models.

% \sunandita{Do we also want to talk about adversarial attacks on time series forecasting in general? such as, \cite{xu2021adversarial}} \biplav{Yes, we should - please add}
% \kl{I added it.}


% ----
\subsection{Robustness Testing of Time-series Forecasting Models}
\cite{gallagher2022investigating} examines the impact of different attacks %; Fast Gradient Signed Method (FGSM), a Single Value, and a label Flip attack, 
on the performance of Convolutional Neural Network model used for time series classification. \cite{pialla2023time} introduces a stealthier attack using the Smooth Gradient Method (SGM) for time series and measures the effectiveness of the attack.
% show ways to detect the attack and make time-series forecasting models robust against such attacks. 
% \cite{wu2022small} show that small perturbations are enough to fool a model. 
% We also explore one such attack called `Saturation change' which is a stealthy attack that is even more harder to detect through visual inspection. 
While \cite{pialla2023time} focuses on measuring the smoothness of the attacks, our work quantifies their impact on the models in addition to the biases they create in models' predictions. \cite{govindarajulu2023targeted} adapt attacks from the computer vision domain to create targeted adversarial attacks. They examine the impact of the proposed targeted attacks versus untargeted attacks using statistical measures. 
% \cite{yoon2022robust} discusses probabilistic time series forecasting in which they extend randomized smoothing techniques to attain robust probabilistic forecasters against certain classes of adversarial perturbations. 
All these works measure the models' performances under perturbations using statistical methods but do not measure the isolated impact of perturbations which is only possible through causal analysis. Furthermore, they do not consider any transformer-based or multi-modal models for evaluation.


\subsection{Causal Analysis in Time-series Forecasting}
\cite{moraffah2021causal} provides a review of the approaches used to compute treatment effects and also discusses causal discovery methods along with commonly used evaluation metrics and datasets. In this paper, they classify the task of estimating the effect of a treatment into three types: (a) Time-varying, (b) Time-invariant, and (c) Dynamic regimes. As the perturbations we apply to our data do not occur at the same timestep in each sample, the effect we are measuring can be considered as time-varying perturbation effect which is more complex to measure compared to time-invariant treatment effects. \cite{robins1999estimation} measures the causal effect of one such time-varying exposure. However, they only consider binary outcomes. In our work, we deal with continuous outcome attribute. \cite{bica2020time} proposes a time series deconfounder which deals with multiple treatment assignments over time and also takes into account hidden confounders. In contrast, we deal with one treatment at a time and focus on analyzing the treatment effects with respect to confounders that are of interest in the time-forecasting domain. 
% Causal Discovery algorithms \cite{zanga2022survey} are generally used when a lot of attributes are involved in a system and if we are interested in finding out the causal relationships between each of these. However, 
% In our work, we focus on only three attributes: 2 types of confounders and one perturbation attribute. We use a hypothesis testing approach to test the validity of each causal link which is simpler and efficient within our experimental setup. 

% \marco{An interesting piece of related work using probabilistic graphical models is~\cite{alsuwat2023malware}, at \url{https://cdn.techscience.cn/files/cmc/2023/TSP_CMC-75-2/TSP_CMC_35126/TSP_CMC_35126.pdf}, which is based on work that the first and third author did for their Ph.D. at South Carolina.}

\subsection{Rating AI Systems}
In the past, there were several works on assessing and rating different AI systems for trustworthiness from a third-party perspective (without access to the system's training data). In \cite{srivastava2018towards,srivastava2020rating,srivastava2023advances-rating}, the authors propose an approach to rate automated machine language translators for gender bias. Further, they create visualizations to communicate ratings \cite{bernagozzi2021vega}, and conduct user studies to determine how users perceive trust \cite{bernagozzi2021vega}. Though they were effective, they did not provide any causal interpretation. In another series of works \cite{kausik2022why, kausik2024rating, kausik2023the}, the authors introduced an approach to rate sentiment analysis systems for bias through causal analysis. 
% using both synthetic and human-generated datasets. 
We extend their method to rate MM-TSFM for robustness against perturbations. There are several advantages of using causal analysis over statistical analysis: causal models allow us to determine accountability and they align well with humanistic values.
% , and also spark collaboration with social sciences leading to the construction of better bias quantification metrics \cite{carey2022causal}. 
Furthermore, they help us quantify the direct influence of various attributes on forecasting accuracy, isolating specific impacts, and mitigating confounding effects.

% \parisa{Also would be great if we highlight why casual analysis are import for this analysis}

% \parisa{maybe some related work on the robustness}

==> AIES2024/sections/conclusion.tex <==
\section{Conclusion}
% \sunandita{I took a pass at the conclusion. Please review and update}
Our study introduces a causal analysis-based method for rating the robustness of Multimodal Time-Series Forecasting Models (MM-TSFM). We extend perturbation techniques to the MM-TSFM domain and evaluate their impact across six different perturbation settings, across industry and company. Notably, our findings highlight the disruptive nature of semantic perturbations, emphasizing the need for robustness evaluations beyond just accuracy metrics. We also find that the variant of ViT-num-spec model trained on a smaller but recent dataset is more robust against compositional perturbation compared to its larger variant. We also find that considering \textit{Industry} as the sensitive attribute / confounder led to an increase in bias compared to \textit{Company}. Moreover, our evaluation shows the commendable performance of ViT-num-spec models, which not only exhibited high accuracy but also demonstrated notable resilience across diverse experimental conditions compared to a traditional numerical baseline. Thus, within the scope of our experiments, multi-
modal (numeric+visual) forecasting exhibit greater robustness compared to simply numeric forecasting. 
% \sunandita{Added the last sentence. Please check.} 
Our rating system provides a practical tool for stakeholders to select robust solutions tailored to their specific data and operational requirements. 

==> AIES2024/sections/discussion.tex <==
\section{Discussion}
Our paper aimed to measure the impact of perturbations and confounders on the outcome of MM-TSFM.  We used the stock prices of six leading companies across three industries for our evaluation. 
% \textit{Though bigger datasets like S\&P 500 or Nasdaq-100 could be used for evaluation, they do not have any confounders that could be easily observed as they just represent stock market indices rather than individual stock prices of companies.}\zhen{I would recommend cutting this out, reviewers could question on why not using the constituents of S\&P 500}  
However, we would like to collect historical data for more than two companies in each industry as future work. The analyses we did in the paper were with respect to \textit{Industry} and \textit{Company}. The motivation behind choosing these specific confounders is based on our intuition that, as stakeholders like investors and analysts are relying more on learning-based systems to decide whether to purchase stocks from a company, they would be interested to know if the errors committed by these learning-based models depend on the range of stock prices (which could serve as a proxy for the industry or company). For example, is a model committing more errors when predicting the stock prices for META compared to MRK? Errors can be committed by other factors such as the volatility of stock prices within an industry. To minimize the effect of volatility, we also performed intra-industry along with inter-industry analysis. As a part of future work, we would also like to do causal analysis considering other confounders such as seasonal trends and additional external factors also be done using additional sources such as financial news. 

As transformer-based approaches and especially multi-modal transformer-based approaches have been proven to be more efficient and accurate compared to traditional uni-modal neural network-based architectures \cite{liu2023survey}, we tested the robustness of one such model that was proved to be more effective for stock price prediction compared to other approaches \cite{zeng2023from}. 

The metrics we have chosen perfectly answered the research questions stated in Section \ref{sec:problem}. Instead of relying on just statistical accuracy metrics as the only performance metrics, we believe that one should select the metrics based on the questions one wants to answer. The hypothesis testing approach introduced in \cite{kausik2024rating}, which we have adapted for our work not only helped us answer the research questions but also quantified the biases and perturbation impacts on the outcome of the test systems. Traditional explainability approaches or other statistical approaches take control from human decision-makers, limiting their involvement \cite{miller2023explainable}. \cite{miller2023explainable} argues that hypothesis-driven decision support, though increases human cognitive load, can truly improve AI-assisted decision support. These approaches usually follow the process of abductive reasoning which involves forming hypotheses and judging their likelihood for explaining the systems' behavior to the end-users. Similarly, in our work, though we initially built a causal model based on our intuition, we tested the validity of each causal link by forming hypotheses and verifying their plausibility through the computation of different metrics. 

Each of the perturbations we used for our analysis has a real-world impact. Some of these could be applied to just numeric data and some can be applied to multi-modal data.  Methods like differential evaluation can be used to find the most impactful variation of a perturbation. But we only aimed to assess whether simple, and sometimes subtle perturbations would have an impact on the outcome of a time-series forecasting model. 

% Each of the tests we performed can be compared to different critics evaluating the models across different distributions and on various aspects, including statistical bias, confounding bias, perturbation impact, and accuracy. By considering all critiques, we reach a common consensus that will be in the form of a rating that could eventually help an end-user decide whether they could trust the system based on the data at hand. 


% \cite{zhou2023explain} -- justification paper. 
% \kl{Significance of Treatment-1. These kind of perturbations can exist in the real-world even if it is simple. We are just testing the stability of the system against these perturbations. Also, how can different combinations of hypotheses can lead to a common conclusion? Breadth and depth of perturbations. Max or average or min of residuals}



% \begin{itemize}
%     \item  Data considered, how to extend to others
%     \item  Multi-modal considered, how to extend to others
%     \item Perturbations considered, how to extend to others
%     \item Metrics considered, how to extend to others
%     \item Confounders considered
% \end{itemize}

==> AIES2024/sections/experiments.tex <==
\section{Experiments and Analysis}
In this section, we describe the experimental apparatus that was used to perform the experiments. It includes the description of test systems, evaluation/test data, and evaluation metrics. We also state and prove certain hypotheses that help us answer the research questions stated in Section \ref{sec:problem}.
\subsection{Experimental Apparatus}
\subsubsection{Test Systems Considered}
We evaluated the following time-series forecasting systems for robustness:

\noindent (a) \textbf{ViT-num-spec}($S_v$): We trained two models on the daily stock time series of S\&P 500 constituents: one using data from before the COVID-19 outbreak and another with data from during the pandemic. We assessed our methodologies by comparing predictions from these models, each trained on datasets from distinct time periods.

\noindent(i) \textbf{ViT-num-spec trained on pre-COVID data  ($S_{v1}$):} The pre-COVID model was trained using 46,875 time series and validated on a separate set of 46,857 time series, spanning from 2000 to 2014. The vision transformer encoder outputs a latent embedding vector with a dimensionality of 128. Training involved a batch size of 128 and employed the AdamW optimizer with a weight decay of 0.05. The process spanned up to 200 epochs, incorporating an early stopping mechanism set with a patience of 10 epochs. Additionally, the base learning rate and learning rate scheduler hyperparameters were finely tuned for the dataset to optimize performance.

\noindent(ii)\textbf{ViT-num-spec trained on during-COVID data ($S_{v2}$)}: 
% \kl{Rachneet / Zhen, can you add some training details here?}
The during-COVID model was trained on a dataset comprising 7,478 time series, and validated on a separate set of 7,475 time series, covering the period from March 2020 to November 2022. It shares the same architecture and parameter tuning routine as the model trained on pre-COVID data, utilizing 80 past time steps to predict the subsequent 20 steps.

\noindent(b) \textbf{ARIMA} ($S_a$): ARIMA (AutoRegressive Integrated Moving Average) model is a widely used statistical approach for time series forecasting. It combines three different components: Autoregressive (AR), differencing (I), and moving average (MA) to capture the patterns in the time-series data and predict the next `d' (from section \ref{sec:problem}) values. To make the time-series data stationary, we had to difference it once. Using ACF and PACF plots, we were able to identify the optimal p and q values. %We used the model to get next 20 (d) stock prices based on the previous 80 (n) stock prices.

\noindent(c) \textbf{Biased system} ($S_b$): We built this system as an extreme baseline. $S_b$ is more biased towards META and GOOG (technology companies) compared to other companies. The system assigns a residual of `0' and `200' for META and GOOG, respectively, while assigning higher residuals to other companies. This ensures that the system shows maximum amount of bias in each setting we considered, representing an extreme baseline for evaluating the performance of other systems. 

\noindent(d) \textbf{Random system} ($S_r$): We built this system as another extreme baseline. $S_r$ assigns random price predictions within the range [MIN(company's stock prices) - 100, MAX(company's stock prices) + 100] based on each company's stock prices. Although the values generated depend on the range of the stock prices for each company, considering the residuals as the outcome, will still add sufficient randomness to the generated numbers. It will also ensure that the random values are contextually meaningful.


\subsubsection{Evaluation/Test Data}
We collected daily stock prices from Yahoo! Finance for six companies: Meta Platforms, Inc. (META), Google (GOO), Pfizer Inc. (PFE), Merck (MRK), Wells Fargo (WFC), and Citigroup Inc. (C). %\biplav{Update to 6 used now.} \sunandita{fixed} 
These companies belong to different sectors with META, GOO in social technology, PFE, MRK in pharmaceuticals, and WFC, C in financial services. The data spans from March 28, 2023, to April 22, 2024. We used a subset of this data, from March 28, 2023, to March 22, 2024, to predict stock prices for the following month. These companies, with their high stock prices, are representative of their respective industry. We applied the sliding window ($width=1$) technique to sample (input, output) pairs for the prediction task. Specifically, the input time series contains 80-days stock prices, and the output contains 20-days stock prices (here, n=80 and d=20 (from section \ref{sec:problem})). %Each new row in the dataset comprises 79 values from the previous row plus one new value.

%Each test system takes in 80 time steps as input and predicts the subsequent 20 steps (here, n=80 and d=20 (from section \ref{sec:problem}))

\subsection{Evaluation Metrics}
\label{sec:metrics}
% \sunandita{Added an intro to this section. Please check.}\kl{Looks good. Thank you.} 
In this section, we define our evaluation metrics. We adapt WRS metric originally proposed in \cite{kausik2024rating}. Additionally, we introduce two new metrics: APE and PIE \% (modified versions of ATE \cite{abdia2017propensity} and DIE \% \cite{kausik2024rating}) tailored to answering RQ2 and RQ3.

\noindent{\bf Weighted Rejection Score (WRS):} WRS was introduced in \cite{kausik2024rating} as a way to measure statistical bias. First, Student's t-test \cite{student1908probable} is used to compare different max residual distributions $(R^{max}_{t} | Z)$ for different values of protected attribute, $Z$. In our case, we measure this between each pair of industries or companies resulting in $^3C_2 = 3$ comparisons. 
%\biplav{Update - just say the count: 6C2 = 15 comparisons?} 
Next, the computed t-value of each pair of companies is compared with the critical t-value 
(computed based on confidence interval (CI) and degrees of freedom (DoF)). Based on this, the null hypothesis is either rejected or accepted. 

    The t-value is computed using the following equation:
    $$t = (mean(x_1) - mean(x_2))/\sqrt{((s_1^2/n_1)+(s_2^2/n_2))}$$

    where $x_1$ and $x_2$ are two $(R^{max}_{t} | Z)$ distributions, $s_1$ and $s_2$ are their standard deviations, and $n_1$, $n_2$ are the sample sizes. %\sunandita{changed count to sample sizes}.  
    \cite{kausik2024rating} added a small $\epsilon$ value to the denominator in cases to handle cases where standard deviation becomes zero. They chose different confidence intervals (CI) [95\%, 75\%, 60\%] that have different critical values and if the computed t-value is less than the critical value, the null hypothesis was rejected. WRS is mathematically defined by the following equation:

    % {\bf Weighted Rejection Score (WRS)} 
    %     \begin{equation}
    %     \begin{split}
    %            = \sum_{i} w_i*x_i
    %     \end{split}
    %     \label{eq:wrs}
    %     \end{equation}

\begin{equation}
\textbf{Weighted Rejection Score (WRS)} = \sum_{i\in CI} w_i*x_i,
\label{eq:wrs}
\end{equation}
    %\sunandita{Added that $i\in CI$. Is that correct?}
    \noindent where, $x_i$ is the variable set based on whether the null hypothesis is accepted (0) or rejected (1). $w_i$ is the weight that is multiplied by $x_i$ based on the CI. For example, if CI is 95\%, $x_1$ is multiplied by 1. The lower the CI, the lower the weight will be. WRS helps us answer RQ1 (see Section~\ref{sec:problem}). 
    \vspace{0.2cm}
    
% \noindent{\bf Deconfounding Impact Estimation (DIE \%):} DIE \% gives us the relative difference between deconfounded and confounded distributions, (Outcome$|$Treatment) i.e., ($\overline{R}_t | T$) in the presence of confounder, `Z'. It was introduced in \cite{kausik2024rating} and is given by the following formula: 

%     {\bf DIE \%} = 
%     {\small
%         \begin{equation}
%         \begin{split}
%         {\frac{ [|E(R^{max}_{t}  =  j| do(P = i)) - E(R^{max}_{t} = j| P = i) | ]} 
%           {E(R^{max}_{t} = j | P = i) }}     * 100
%         \label{eq:die}
%         \end{split}
%         \end{equation}
%     }

% Here, $P = 0$ is control,  $P = i, i \in $ \{1,5\} any  perturbation, and $j$ is the outcome/residual.
%     The higher the DIE \%, the greater the confounding bias present in the system. %\sunandita{TODO: add what is j}

\noindent{\bf Average Perturbation Effect (APE)}: Average Treatment Effect (ATE) provides the average difference in outcomes between units in the treatment and units in the control \cite{wang2017g}. In our context, it computes the difference between residuals between perturbed data points (P1 through P5) and the data points in the control (P0). Hence, we refer to this metric as APE. This metric helps us answer RQ3. It is formally defined using the following equation:

    {\bf APE} = 
    {\small
        \begin{equation}
        \begin{split}
        [|E[R^{max}_{t} = j| do(P = i)] - E[R^{max}_{t} = j| do(P = 0)]| ]
        \label{eq:ape}
        \end{split}
        \end{equation}
    } 

    
    % where $P = 0$ is the control group and $P = i$ can be any applied perturbation.
    
\noindent {\bf Propensity Score Matching - Deconfounding Impact Estimation \% (PSM-DIE \% or in short, PIE \%):} In \cite{kausik2024rating}, the authors used a linear regression model to estimate the causal effects. This model assumes that the relationship between the treatment variables, covariates, and outcome is linear. The linear regression method does not capture non-linear relationships and may not fully eliminate confounding biases. They proposed a metric called DIE \% that computes relative difference between deconfounded and confounded distributions using binary treatment values. However, we use six different treatment (or perturbation) values in our work. We use the Propensity Score Matching (PSM) \cite{rosenbaum1983central} technique that specifically targets the confounding effect by matching the treatment and control units based on the probability of receiving a treatment, making both groups comparable. PSM is analogous to randomized controlled trials (RCTs) and does not involve the outcome variables \cite{baser2007choosing}, whereas linear regression does. We modify DIE \% and introduce the PIE \% (PSM-DIE\%) metric. This metric helps us answer RQ2. It is given by the formula:

   % {\bf PIE \%} = 
    {\small
        \begin{equation}
        \textbf{PIE \%} = \left[ ||APE_{o}| - |APE_{m}|| \right] * 100
        \label{eq:pie}
        \end{equation}
    }
    
   $APE_{o}$ and $APE_{m}$ represent the APE computed before and after applying PSM respectively. $PIE \%$ computes the true impact $Z$ has on the relation between $P$ and $R^{max}_{t}$.

% \kl{SMAPE, MASE, Sign Accuracy}

\noindent {\bf Symmetric mean absolute percentage error (SMAPE) } is defined as, 
    {\small
    \begin{equation} \label{eq:smape}
        SMAPE = \frac{1}{T}\sum_{t=1}^T\frac{|x_t - \hat{x}_t|}{(|x_t| +|\hat{x}_t|)/2}, 
    \end{equation}
    }
where $T= 20$ is the total number of observations in the predicted time series, $x_t$ represents the actual observed values, and $\hat{x}_t$ the predicted values at each time step $t= 1, \ldots, 20$. SMAPE scores range from 0 to 2, with lower scores indicating more precise forecasts. 

\noindent {\bf Mean absolute scaled error (MASE)} quantifies the mean absolute error of the forecasts relative to the mean absolute error of a naive one-step forecast calculated on the training data.
{\small
\begin{equation}\label{eq:mase}
    MASE=\frac{\frac{1}{T} \sum_{i=t+1}^{t+T}|x_{i} - \hat{x_{i}}|}{\frac{1}{t}\sum_{i=1}^{t}|x_{i} - x_{i-1}|},
\end{equation}
}
where in our case, $t = 80$, and $T = 100$.
Lower MASE values indicate better forecasts. 

\noindent {\bf Sign Accuracy} quantifies the average classification accuracy across all test samples, where a higher accuracy indicates more precise predictions. This metric classifies based on how the predicted forecasts align with the most recent observed values in the input time series.
% We categorize forecast movements into three distinct classes: class 1 represents ``going up," class 2 denotes ``remaining flat," and class 3 signifies ``going down." 

\subsection{Experimental Evaluation}
\label{sec:expts}
% All the experiments are designed to bring out the worst possible behavior of different systems. 
% The following four hypotheses answer the research questions stated in Section \ref{sec:problem}. 
In this section, we state hypotheses, the experimental setup used, the results obtained, interpretations made from the results, and the conclusions drawn from the interpretations. Table \ref{tab:cases} summarizes the research questions answered through the hypotheses stated along with the corresponding causal diagrams and key findings from these hypotheses. Some of the experimental results can be found in the supplementary. Table 3 and 4 in the supplementary show partial order and final order with respect to WRS, APE, SMAPE, and Sign Accuracy.

\begin{table*}[ht]
\centering
   {\tiny
    \begin{tabular}{|p{14em}|p{12em}|p{14em}|p{4em}|p{30em}|}
    \hline
          {\bf Research Question} &    
          {\bf Hypothesis} & 
          {\bf Causal Diagram} &
          {\bf Metrics Used} &
          {\bf Findings} \\ \hline 
          
          \textbf{RQ1:} Does $Z$ affect $R^{max}_{t}$ of $S$, even though $Z$ has no effect on $P$? & 
          \emph{Company} affects the \emph{Residual} of \emph{S}, even though \emph{Company} has no effect on \emph{Perturbation}. &
          \begin{minipage}{.05\textwidth}
          \vspace{2.5mm}
          \centering
          \includegraphics[width=30mm, height=15mm]{figs/Causal_H1.png}
          \end{minipage} &
          WRS &
          (Table 2 and 3 in the supplementary) \textbf{\textit{S} with low statistical bias}: $S_a$ and $S_{v2}$. \textbf{\textit{P} that led to more statistical bias}: P1 and P2.  \textbf{Analysis with more discrepancy}: Inter-industry
          \\ \hline 
          % -------
          \textbf{RQ2:} Does $Z$ affect the relationship between $P$ and $R^{max}_{t}$ of $S$ when $Z$ has an effect on $P$?& 
          \emph{Company} affects the relationship between \emph{Perturbation} and \emph{Residual} of \emph{S} when \emph{Company} has an effect on \emph{Perturbation}. &
          \begin{minipage}{.05\textwidth}
          \vspace{2.5mm}
          \centering
          \includegraphics[width=30mm, height=15mm]{figs/Causal_H2.png}
          \end{minipage} &
          PIE \% &
          (Table 2 in supplementary and Table \ref{tab:ratings-pie}) \textbf{\textit{S} with low confounding bias}: $S_{v2}$ and $S_{v1}$. \textbf{\textit{P} that led to more confounding bias}: P1 and P2.  \textbf{Confounder that led to more bias}: \textit{Industry}
          \\ \hline 
          % -------
          \textbf{RQ3:} Does $P$ affect $R^{max}_{t}$ of $S$ when $Z$ has an effect on $P$? & 
          \emph{Perturbation} affects the \emph{Residual} of \emph{S} when \emph{Company} has an effect on \emph{Perturbation}. &
          \begin{minipage}{.05\textwidth}
          \vspace{2.5mm}
          \centering
          \includegraphics[width=30mm, height=15mm]{figs/Causal_H3.png}
          \end{minipage} &
          APE &
          (Table 2 and 4 in the supplementary) \textbf{\textit{S} with low APE}: $S_{v1}$. \textbf{\textit{P} with high APE}: P1 and P2.  \textbf{Confounder that led to high APE}: \textit{Industry}
          \\ \hline 
          % -------
          \textbf{RQ4:} Does $P$ affect $\hat{Y_{t}}$ of $S$ in the presence of $P$? & 
          Semantic and compositional \emph{Perturbations} can degrade the performance of \emph{S}.  &
          This hypothesis does not necessitate a causal model for its evaluation. &
          SMAPE, MASE, Sign Accuracy &
          (Table \ref{tab:h4}) \textbf{\textit{S} with good performance}: $S_{v1}$. \textbf{\textit{P} with high impact on performance}: P1, P2 and P5.  
          \\ \hline 
    \end{tabular}
    }
    \caption{Summary of the research questions answered in the paper along with corresponding hypotheses stated, causal diagram, metrics used in the experiment, and the important findings from the experiment.
    %\zhen{shall we still include Z, P, R in the column of causal diagram like in Figure 1? to keep it directly relatable to the RQs?}
    }
    \label{tab:cases}
\end{table*}


\begin{table}[!ht]
\centering
{\tiny
    \begin{tabular}{|p{4.5em}|p{0.5em}|p{15em}|p{12em}|}
    \hline
          {\bf Forecasting Evaluation Dimensions} &
          {\bf P} &    
          {\bf Partial Order} &
          {\bf Complete Order} 
          \\ \hline 
          \multirow{5}{6em}{Confounding Bias with \textit{Industry} as confounder (PIE$_I$ \%)} &
          P1 & 
          \{$S_{v1}$: 630.10, $S_a$: 982.38, $S_{v2}$: 1191.91, $S_r$: 4756.40,  $S_b$: 6916.11\} &
          \{\textbf{S$_{v1}$: 1}, $S_a$: 1, $S_{v2}$: 2, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P2 & 
          \{$S_{v1}$: 941.93, $S_a$: 1275.04, $S_{v2}$: 1490.65, $S_r$: 4274.38,  $S_b$: 9474.61\} &
          \{\textbf{S$_{v1}$: 1}, $S_a$: 1, $S_{v2}$: 2, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P3 & 
          \{$S_{v2}$: 224.98, $S_{v1}$: 276.86, $S_r$: 3560.94,  $S_b$: 7489.48\} &
          \{\textbf{S$_{v2}$: 1}, $S_{v1}$: 1, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P4 & 
          \{$S_{v1}$: 229.03, $S_{v2}$: 1694.57, $S_r$: 2250.35,  $S_b$: 7618.25\} &
          \{\textbf{S$_{v1}$: 1}, $S_{v2}$: 1, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P5 & 
          \{$S_{v2}$: 273.12, $S_{v1}$: 344, $S_r$: 4025.31,  $S_b$: 8966.57\} &
          \{\textbf{S$_{v2}$: 1}, $S_{v1}$: 1, $S_r$: 2,  $S_b$: 3\} 
          \\ \hline
          \multirow{5}{6em}{Confounding Bias with \textit{Company} as confounder (PIE$_C$ \%)} &
          P1 & 
          \{$S_{v2}$: 415.74, $S_{v1}$: 551, $S_a$: 914.64, $S_r$: 1041.01,  $S_b$: 3283.88\} &
          \{\textbf{S$_{v2}$: 1}, $S_{v1}$: 1, $S_a$: 2, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P2 & 
          \{$S_{v2}$: 575.12, $S_{v1}$: 898.90, $S_a$: 1154.87, $S_r$: 1463.71,  $S_b$: 2174.39\} &
          \{\textbf{S$_{v2}$: 1}, $S_{v1}$: 1, $S_a$: 2, $S_r$: 2,  $S_b$: 3\} 
          \\\cline{2-4}
          &
          P3 & 
          \{$S_{v2}$: 1277.44, $S_r$: 1305.78,   $S_b$: 1846.56, $S_{v1}$: 2427.35\} &
          \{\textbf{S$_{v2}$: 1}, $S_r$: 1, $S_b$: 2,  $S_{v1}$: 3\} 
          \\ \cline{2-4}
          &
          P4 & 
          \{$S_{v1}$: 247.80, $S_{v2}$: 942.02, $S_r$: 1314.82,  $S_b$: 3557.45\} &
          \{\textbf{S$_{v1}$: 1}, $S_{v2}$: 1, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P5 & 
          \{$S_{v2}$: 284.95, $S_{v1}$: 378.19, $S_r$: 1928.21,  $S_b$: 2118.88\} &
          \{\textbf{S$_{v2}$: 1}, $S_{v1}$: 1, $S_r$: 2,  $S_b$: 3\} 
          \\\hline
          \multirow{5}{6em}{Accuracy (MASE)} &
          P0 & 
          \{$S_{v1}$: 3.68, $S_a$: 3.79, $S_{v2}$: 3.89, $S_r$: 86.45,  $S_b$: 947.56\} &
          \{\textbf{S$_{v1}$: 1}, $S_a$: 1, $S_{v2}$: 2, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P1 & 
          \{$S_{v1}$: 5.30, $S_{v2}$: 11.18, $S_a$: 18.36, $S_r$: 86.99,  $S_b$: 947.56\} &
          \{\textbf{S$_{v1}$: 1}, $S_{v2}$: 1, $S_a$: 2, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P2 & 
          \{$S_{v1}$: 4.24, $S_{v2}$: 6.16, $S_a$: 8.24, $S_r$: 86.87,  $S_b$: 947.56\} &
          \{\textbf{S$_{v1}$: 1}, $S_{v2}$: 1, $S_a$: 2, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P3 & 
          \{$S_{v1}$: 3.68, $S_{v2}$: 3.89, $S_r$: 86.65,  $S_b$: 947.56\} &
          \{\textbf{S$_{v1}$: 1}, $S_{v2}$: 1, $S_r$: 2,  $S_b$: 3\} 
          \\\cline{2-4}
          &
          P4 & 
          \{$S_{v1}$: 3.67, $S_{v2}$: 3.90, $S_r$: 86.53,  $S_b$: 947.56\} &
          \{\textbf{S$_{v1}$: 1}, $S_{v2}$: 1, $S_r$: 2,  $S_b$: 3\} 
          \\ \cline{2-4}
          &
          P5 & 
          \{$S_{v2}$: 3.93, $S_{v1}$: 8.26, $S_r$: 87.20,  $S_b$: 947.56\} &
          \{\textbf{S$_{v2}$: 1}, $S_{v1}$: 1, $S_r$: 2,  $S_b$: 3\} 
          \\ \hline
    \end{tabular}
    }
    \caption{Final raw scores and ratings based on PIE \% and MASE. Higher rating indicate higher bias (or error, for MASE). For simplicity, we denoted the raw scores for MASE using just the mean value, but standard deviation was also considered for rating. The chosen rating level, L = 3. From P1 and P2 results, it can be observed that for S$_{v1}$ the PIE$_I$ is almost 30 \% lower and MASE is 60 \% lower on average compared to $S_a$.}
    \label{tab:ratings-pie}
\end{table}
%\vspace{-1em}

{\color{blue}\noindent{\bf Hypothesis-1:}} \emph{Sensitive Attribute} affects the \emph{Residual} of \emph{S}, even though \emph{Sensitive Attribute} has no effect on \emph{Perturbation}.

\noindent{\bf Experimental Setup:}
In this experiment, the causal link from the \emph{Sensitive Attribute} to \emph{Perturbation} will be absent as the application of perturbation to the stock prices does not depend on the corresponding company name or the industry i.e., perturbations are applied uniformly across all the data points. The corresponding causal diagram is shown in table \ref{tab:cases}. We quantify the statistical bias exhibited by the systems by using WRS that was defined in equation \ref{eq:wrs}. To compare \emph{Residual} distributions across different \emph{Sensitive Attribute} stock prices, we use t-value, p-value, and DoF from the Student's t-test \cite{student1908probable} to compare different outcome distributions across each of the companies. We perform two different analyses in this experiment: one to measure the discrepancy $S$ shown across different industries (WRS$_{Industry}$) and another to measure the discrepancy $S$ among both the companies (WRS$_{Company}$) within the same industry.  





\noindent{\bf Results:} Table 1 in the supplementary shows the t-statistic computed for all distributions along with the number of rejections under each confidence interval and Table 2 in the supplementary shows the Weighted Rejection Scores (WRS) across companies within the same industry (WRS$_I$) and different industries (WRS$_C$) that quantify the statistical bias exhibited by different test systems. The final ratings with respect to the WRS are shown in Table 3 in the supplementary.

\noindent{\bf Interpretation:}  From Table 2 in the supplementary, most discrepancies can be observed across industries compared to the discrepancies across companies i.e., all the test systems make more prediction errors when compared across different industries. When the input data was subjected to perturbations P1 and P2, the systems exhibited more statistical bias. From Table 3 in the supplementary, $S_{v2}$ and $S_a$ exhibited the least amount of statistical bias under most of the perturbations compared to other systems. 

\noindent{\bf Conclusion:} $S_a$ and $S_{v2}$ outperformed other systems in terms of statistical bias. Systems exhibited more bias when P1 and P2 were applied and showed more statistical bias when compared across different industries rather than different companies within the same industry. Hence, \emph{Sensitive Attribute} affects the \emph{Residual} of \emph{S}, even though \emph{Sensitive Attribute} has no effect on \emph{Perturbation}. 

{\color{blue}\noindent{\bf Hypothesis-2:}} \emph{Confounder} affects the relationship between \emph{Perturbation} and \emph{Residual} of \emph{S} when \emph{Confounder} has an effect on \emph{Perturbation}.


\noindent{\bf Experimental Setup:} In this experiment, we use PIE \% defined in equation \ref{eq:pie} to compare the APE (defined in equation \ref{eq:ape}) before and after deconfounding using the Propensity Score Matching (PSM) technique as the presence of the confounder opens a backdoor path from \emph{Perturbation} to  \emph{Residual} through the \emph{Confounder}. The causal link from \emph{Confounder} to \emph{Perturbation} will be valid only if the perturbation applied depends on the value of the confounder (i.e. the company or the industry the specific data points belong to). To ensure the probability of perturbation assignment varies with respect to the \emph{Confounder} across three distributions (DI1 through DI3) in the case of \emph{Industry} and six different distributions in the case of \emph{Company} (DC1 through DC6), we implemented weighted sampling. For each distribution, weights were configured so that perturbation groups P1 through P5 had a twofold higher likelihood of selection compared to P0 for specific values of the confounder. For example, META in DC1, GOOG in DC2, and so on. This strategy highlights significant cases, although other combinations are possible for further exploration. Computing APE involves the following steps: First, we use logistic regression to estimate the probability of each data point receiving the perturbation based on the company or the industry it belongs to. Next, we match each perturbed data point with a control (not perturbed) data point that was not perturbed but has a similar probability of having perturbed. This matching process ensures that both groups are comparable, allowing us to isolate and measure the actual impact of the perturbation. 


\noindent{\bf Results:}
Table 2 in the supplementary shows the PIE$_C$ \% (when \textit{Company} acts as the confounder) and PIE$_I$ \% (when \textit{Industry} acts as the confounder) values computed for different systems across different distributions. As our rating method aims to bring the worst possible behavior of the systems, we take the MAX(PIE\%) (highlighted in bold in Table 2 in the supplementary) as the raw score that is used to compute the final ratings shown in Table \ref{tab:ratings-pie}. Each of the values in the tuple in PIE \% shows the difference between APE before and after propensity score matching for different distributions. In each case, P0 is considered as the control group.


\noindent{\bf Interpretation:} From Table 2 in the supplementary, in most cases, choosing \textit{Industry} as the confounder led to more confounding bias in the systems. From Table \ref{tab:ratings-pie}, $S_{v2}$ and $S_{v1}$ exhibited the least amount of confounding bias with $S_{v2}$ outperforming all other systems in most cases. In most cases, systems exhibited more confounding bias when perturbations P1 and P2 were applied with P4 having the least impact and did not exacerbate the confounding bias significantly.  

\noindent{\bf Conclusion:} \textit{Industry} showed higher confounding bias. Both $S_{v1}$ and $S_{v2}$ performed better than all the systems, with $S_{v2}$ being the least biased of all. However, even they show some confounding bias. P1 and P2 proved to be the most impactful perturbations that led to more confounding bias. Hence, \emph{Confounder} affects the relationship between \emph{Perturbation} and \emph{Residual} of \emph{S} when \emph{Confounder} has an effect on \emph{Perturbation} which leads to confounding bias.

{\color{blue}\noindent{\bf Hypothesis-3:}} \emph{Perturbation} affects the \emph{Residual} of \emph{S} when \emph{Company} has an effect on \emph{Perturbation}.


\noindent{\bf Experimental Setup:}
The experimental setup in this experiment is same as that for Hypothesis-2. To compute the APE, we used PSM, the steps of which were detailed in the experimental setup of Hypothesis-2. PSM allows us to effectively determine the effect of \emph{Perturbation} on the \emph{Residual}. For instance, if two matched points belong to the same company but only one was perturbed, any difference in their residuals can be directly attributed to the perturbation itself rather than to other confounding factors. This method provides a clear understanding of the true impact of the \emph{Perturbation} on the \emph{Residual}.

\noindent{\bf Results:}
Table 2 in the supplementary shows the APE$_C$ \% (when \textit{Company} acts as the confounder) and APE$_I$ \% (when \textit{Industry} acts as the confounder) values computed for different systems across different distributions after applying PSM. As our rating method aims to bring the worst possible behavior of the systems, we take the MAX(APE) as the raw score (highlighted in bold in Table 2 in the supplementary) that is used to compute the final ratings. Each of the values in the tuple in APE shows the APE after propensity score matching across different distributions. In each case, P0 is considered as the control group. 


\noindent{\bf Interpretation:} It is undesirable to have a higher APE, as it implies that the perturbation applied can have a significant impact on the residuals computed for different systems. From the APE values in Table 2 in the supplementary, when \textit{Industry} was considered as the confounder, it led to a higher APE. As the outcome of $S_b$ depended on the \textit{Company} (and varied from one company to another), the perturbation did not have any effect on the system. Whereas, when \textit{Industry} was considered as the confounder, the perturbation appeared influential, resulting in a high APE.  From Table 4 in the supplementary, perturbations had the least impact on $S_{v1}$ and $S_{v2}$ and more impact on $S_a$ (more than $S_r$). Among all the perturbations, P1 and P2 were the most disruptive.

\noindent{\bf Conclusion:} Perturbations had lesser impact on $S_{v1}$ and higher impact on $S_a$. P1 and P2 were the most disruptive perturbations. Considering \textit{Industry} as the confounder led to higher APE. Overall, \emph{Perturbation} affects the \emph{Residual} of \emph{S} when \emph{Company} has an effect on \emph{Perturbation}.

{\color{blue}\noindent{\bf Hypothesis-4:}} Semantic and compositional \emph{Perturbations} can degrade the performance of \emph{S}. 

\noindent{\bf Experimental Setup:} For this experiment, we do not use the causal model. The metric computation method is statistical. We compute the three accuracy metrics measured in \cite{zeng2023from} and summarized in Section \ref{sec:metrics}. 


\begin{table}
\centering
   {\tiny
    \begin{tabular}{|l|p{0.4em}|p{5em}|p{5em}|p{5em}|p{2em}|p{5em}|}
    \hline
          {\bf Metric} &
          {\bf P} &    
          {\bf $S_{v1}$} &
          {\bf $S_{v2}$} &
          {\bf $S_a$} & 
          {\bf $S_b$} &
          {\bf $S_r$}
          \\ \hline 
          \multirow{6}{1em}{SMAPE$\downarrow$} & 
          P0 &
          \textbf{0.039 $\pm$ 0.035} &
           0.041 $\pm$ 0.037 &
           0.040 $\pm$ 0.037 &
          \multirow{6}{1.5em}{1.276 $\pm$ 0.663} &
          0.829 $\pm$ 0.638
          \\ \cline{2-5}
            \cline{7-7}
          % -------
            & 
          P1 &
          \textbf{0.064 $\pm$ 0.167 }&
          0.127 $\pm$ 0.112 &
          0.084 $\pm$ 0.282 &
          &
          0.830 $\pm$ 0.639
          \\ \cline{2-5}
          \cline{7-7}
          % -------
            & 
          P2 &
          \textbf{0.047 $\pm$ 0.069 }&
          0.068 $\pm$ 0.058 &
          0.069 $\pm$ 0.217 &
          &
          0.830 $\pm$ 0.639
          \\ \cline{2-5}
          \cline{7-7}
          % -------
            & 
          P3 &
          \textbf{0.039 $\pm$ 0.035} &
          0.041 $\pm$ 0.037 &
          NA &
             &
          0.830 $\pm$ 0.640
          \\ \cline{2-5}
          \cline{7-7}
          % -------
            & 
          P4 &
          \textbf{0.039 $\pm$ 0.035} &
          0.041 $\pm$ 0.037 &
          NA &
          &
          0.829 $\pm$ 0.639
          \\ \cline{2-5}
          \cline{7-7}
          % -------
            & 
          P5 &
          0.089 $\pm$ 0.074 &
          \textbf{0.041 $\pm$ 0.035}  &
          NA &
          &
          0.832 $\pm$ 0.635
          \\ \hline
          % -------

          \multirow{6}{1em}{MASE$\downarrow$} & 
          P0 &
          \textbf{3.68 $\pm$ 3.44} &
          3.89 $\pm$ 3.64 &
          3.79 $\pm$ 3.59 &
          \multirow{6}{1em}{947.56 $\pm$ 767.65} &
          86.45 $\pm$ 72.72
          \\ \cline{2-5}
          \cline{7-7}
          % -------
             & 
          P1 &
          \textbf{5.30 $\pm$ 9.60} &
          11.18 $\pm$ 9.42 &
          18.36 $\pm$ 168.82 &
          &
          86.99 $\pm$ 73.53 
          \\ \cline{2-5}
          \cline{7-7}
          % -------
             & 
          P2 &
          \textbf{4.24 $\pm$ 5.56} &
          6.16 $\pm$ 5.16 &
          8.24 $\pm$ 48.58 &
          &
          86.87 $\pm$ 73.32 
          \\ \cline{2-5}
          \cline{7-7}
             & 
          P3 &
          \textbf{3.68 $\pm$ 3.44} &
          3.89 $\pm$ 3.64 &
          NA &
          &
          86.65 $\pm$ 73.11 
          \\ \cline{2-5}
          \cline{7-7}
          % -------
             & 
          P4 &
          \textbf{3.67 $\pm$ 3.43}   &
          3.90 $\pm$ 3.65 &
          NA &
          &
          86.52 $\pm$ 73.07 
          \\ \cline{2-5}
          \cline{7-7}
          % -------
             & 
          P5 &
          8.26 $\pm$ 7.18 &
          \textbf{3.93 $\pm$ 3.54} &
          NA &
          &
          87.20 $\pm$ 73.14 
          \\ \hline
          % -------
          \multirow{6}{2em}{Sign Accuracy (\%)$\uparrow$}   & 
          P0 &
          51.32 &
          51.28 &
          \textbf{60.08} &
          \multirow{6}{1em}{62.60} &
          49.88
          \\ \cline{2-5}
             & 
          P1 &
          48.77 &
          41.54 &
          \textbf{57.08} &
          &
          49.62
          \\\cline{2-5}
             & 
          P2 &
          \textbf{58.69} &
          45.28 &
          57.13 &
          &
          49.64
          \\ \cline{2-5}
              & 
          P3 &
          51.35 &
          \textbf{54.74} &
          NA &
          &
          49.71
          \\ \cline{2-5}
             & 
          P4 &
          \textbf{53.95} &
          51.14 &
          NA &
          &
          49.67
          \\\cline{2-5}
             & 
          P5 &
          43.97 &
          \textbf{52} &
          NA &
          &
          50.05
          \\ \hline
    \end{tabular}
    %}
    \caption{Performance metrics for test systems across different perturbations. SMAPE and MASE scores are reported as mean $\pm$ standard deviation. As P3 through P5 could not be applied to $S_a$, the metric values are marked as `NA'.}
    \label{tab:h4}
    }
\end{table}
\noindent{\bf Results:}
Table \ref{tab:h4} shows the performance metrics (used in \cite{zeng2023from}):
SMAPE, MASE, and Sign accuracy computed for all the test systems across all perturbations. As P3 through P5 could not be applied to $S_a$, we marked the metric values as `NA'. 

\noindent{\bf Interpretation:} For perturbations P1 through P4, $S_{v1}$ outperformed all other systems in terms of SMAPE and MASE. As $S_b$'s residuals vary depending on the ground truth stock prices of specific companies, $S_b$ consistently predicts the correct directional movement of stock prices. After $S_b$ (62.60 \%), $S_a$ shows higher sign accuracy for P0 and P1. For perturbations P2 through P5, the sign accuracies of $S_{v1}$ and $S_{v2}$ do not vary much compared to P0 (sometimes the accuracy exceeds P0). SMAPE and MASE values indicate that the performance of the models degrade when perturbations P1, P2 and P5 are applied compared to P3 and P4.

\noindent{\bf Conclusion:} Hence, semantic and compositional \emph{Perturbations} can degrade the performance of \emph{S}. 

==> AIES2024/sections/introduction.tex <==
\section{Introduction}

Artificial Intelligence (AI) systems, regardless of the mode in which they take input - numeric, textual, audio, visual, or multimodal,  are notorious for their
fragility (lack of robustness) and other characteristics (e.g., opaqueness, alignment to human values) that go beyond performance to contribute to users' trust of technology\cite{trust-ml-book}. For example, small variations in the inputs to a Machine Learning (ML) model may
result in 
% significant and 
drastic swings in its output. 
This uncertainty about robustness is amplified by the lack of interpretability of many ML models due to their black-box nature \cite{explainable-ai-survey}.
As a result, such systems face challenges in gaining acceptance and trust from end-users hampering their widespread adoption.


When such systems are deployed in critical areas like finance \cite{imf-ai-impact-report}
and healthcare \cite{ai-health-report}, the consequences of their uncertain behavior could cause critical failures. A promising idea to manage user trust is to {\em communicate} the behavior of AI systems through ratings that are assigned after assessing AI systems from a third-party perspective (without access to the system's training data). These methods \cite{srivastava2018towards,srivastava2020rating,srivastava2023advances-rating,kausik2023the,kausik2024rating}, have considered text-based AI systems like automated machine translators and sentiment analysis systems in various settings including multi-lingual text, using which it was shown that users can make informed decisions when a choice of AI models are available to them. Along these lines, we consider multimodal data and time-series forecasting-based AI models.

% the authors propose an approach to rate automated machine language translators for gender bias. 
% \sunandita{We needs a sentence here saying what we are adding to the literature. Can we say that while there are existing rating methods for single modal models we focus on multi-modal time series forecasting model? Or something similar} \biplav{Yes - will add.} 

% More specifically, in time-series forecasting, for instance,
Time-series forecasting is a popular form of AI usage in many industries including finance. 
%In time-series forecasting,
Here, imprecision due to noisy or incorrect data can lead to erroneous predictions, impacting stakeholders who rely on AI models for their day-to-day work. Many current models in this domain use multimodal AI systems to predict trends and stock prices due to their effectiveness over numerical data. \cite{zeng2023from} is one such work in which the authors introduced ViT-num-spec MM-TSFM and showed that it outperformed other numerical and image-based models.
Hence, we select daily stock price prediction task to assess various time-series forecasting models including two MM-TSFM that use ViT-num-spec architecture. We collected 13 months of stock prices from six leading companies, two from each of the three critical industries: Technology, Pharmaceuticals, and Finance. We organized this data into 2,75,400 data points
% \zhen{it this number computed as $\#$ of data points per stock over 13 months * 5 * 10 * 6?} 
across five model predictions, ten sampled distributions, and six perturbed variations. 

Our contributions are that we:
%\noindent 
1. Introduce a causal analysis-based method to rate Multimodal Time-Series Forecasting Models (MM-TSFM) for robustness (Section \ref{sec:rating}). 
%\noindent 
2. Extend perturbation techniques used in other contexts to MM-TSFM, demonstrating their impact in three different settings and evaluating their robustness using our rating method across these settings: Input-specific Perturbation (IP), Semantic Perturbation (SP), and Compositional Perturbation (CP) (Section \ref{sec:perturbations}).
%\noindent 
3. Demonstrate how stakeholders can utilize our ratings to choose a resilient MM-TSFM from the available alternatives, considering the data provided (see Table \ref{tab:cases}).
    % \sunandita{rephrased this point and referring to Table 1 instead of table 2. Also moved this point earlier. Please check.}
%\noindent 
4. Find that our rating system suggests that semantic perturbations are the most disruptive compared to other perturbations for all the test systems (Section \ref{sec:expts}). 
% \sunandita{for which systems, only Vit-num-spec or all? Can we quantify the relative difference for the most disruptive perturbation? }
%%
    % \item Find that ViT-num-spec models are not only accurate but also emerged as notably robust across various experimental conditions compared to its numerical baseline (Table \ref{tab:ratings-pie}).  
%\noindent 
5. Within the scope of our study, we conclude that multi-modal forecasting, which combines numeric and visual data and has been previously shown to outperform purely numeric forecasting, exhibit greater robustness as well (Table \ref{tab:ratings-pie}) with MM-TSFM showing 30 \% lower confounding bias and 60 \% lower MASE under semantic perturbations, compared to numerical forecasting.
    % \sunandita{I have added the last sentence. Please check.}
   

In the remainder of the paper, we begin with a background on time-series forecasting and rating of AI systems, followed by the problem formulation and an introduction to our setup, which includes datasets, test systems, and perturbations. We present various hypotheses and support them with experimental results. We conclude with a discussion. The supplementary material contains rating algorithms adapted from \cite{kausik2024rating}, and some additional results.

==> AIES2024/sections/method.tex <==
\section{Method}
In this section, we discuss the architecture and working of MM-TSFM introduced in \cite{zeng2023from}. We then describe the different types of perturbations we used to assess MM-TSFM. We also describe the rating method tailored to our setting, originally introduced in \cite{kausik2024rating}. 

\subsection{Multi-modal Time-series Forecasting Models (MM-TSFM)}
\label{sec:models}
In this study, we employ the $\textbf{ViT-num-spec}$ model \cite{zeng2023from}, which combines a \textbf{\underline{vi}}sion \textbf{\underline{t}}ransformer with a multimodal time-frequency \textbf{\underline{spec}}trogram, augmented by the intensities of \textbf{\underline{num}}eric time series for time series forecasting. This model enhances predictive accuracy by leveraging both visual and numerical data. Specifically, it transforms numeric time series into images using a time-frequency spectrogram and utilizes a vision transformer (ViT) encoder with a multilayer perceptron (MLP) head for future predictions. We trained two variations of the ViT-num-spec model using two real-world datasets and conducted evaluations using a separate dataset.

% We used two real-world datasets to train two variations of the ViT-num-spec model \cite{zeng2023from} and used a separate dataset for model evaluation.
% In this work, we utilize the \textbf{ViT-num-spec} model \cite{zeng2023from}, which integrates a \textbf{\underline{vi}}sion \textbf{\underline{t}}ransformer with a multimodal time-frequency \textbf{\underline{spec}}trogram, augmented by the intensities of \textbf{\underline{num}}erical time series for time series forecasting. The ViT-num-spec method leverages both the visual and numerical data from the spectrogram to enhance predictive accuracy. It transforms numerical time series into images using a time-frequency spectrogram and subsequently employs a vision transformer (ViT) encoder with a multilayer perceptron (MLP) head to predict future time series.\sunandita{are the events predicted or just the impact of these events on the stock prices?} 
% \biplav{Kausik, Zeng, Rachneet: make this into simple sentences. Hard to follow.}

\subsubsection{Time-Frequency Spectrogram} \label{subsec:spectrogram}
Building on the method of \cite{zeng2023from}, we use wavelet transforms \cite{daubechies1990wavelet} to create time-frequency spectrograms from time series data. 
Specifically, we employ the Morlet wavelet (see \cite{morlet2}) with scale $s$, and $\omega_0 = 5$ by default, as detailed in Equation \ref{wavelet_eq}. The parameter $s$ represents the scale of the wavelet, affecting its width and localization in time, while $\omega_0$ is the central frequency of the wavelet, influencing its oscillatory behavior. The wavelet function $\psi(x)$ is given by:
{
\tiny
\begin{equation}
\label{wavelet_eq}
\psi(x) = \sqrt{\frac{1}{s}} \pi^{-\frac{1}{4}} \exp\left(-\frac{x^2}{2s^2}\right) \exp\left(j\omega_0\frac{x}{s}\right)
\end{equation}
}

% Specifically, we employ the Morlet wavelet (see \cite{morlet2}) with scale $s$, Omega0 $w$ with a default value of 5,  detailed in Equation \ref{wavelet_eq} \biplav{explain params of equation}:
% \begin{equation}\label{wavelet_eq}
% \psi(x) = \sqrt{\frac{1}{s}} \pi^{-\frac{1}{4}} \mathrm{e}^{\frac{1}{2}\frac{x}{s}} \mathrm{e}^{jw\frac{x}{s}}
% \end{equation}
This method involves convolving the time series with wavelets at various scales. The magnitudes of the resulting coefficients indicate the strength of the signal at different frequencies. These magnitudes are visualized in a spectrogram, with higher frequencies positioned at the top and lower ones at the bottom. To enhance the utility of these spectrograms, an image stripe is added at the top of the spectrogram image to retain the sign information of the time series. Specifically, this image stripe is converted from the standardized numeric time series, into a stripe of pixels with intensity values ranging from 0 to 255. This enhanced image is then used as the input for the vision transformer model, as discussed next.
% \sunandita{Are we doing anything different from the previous paper here? If so, please highlight.}
% \zhen{To avoid confusion with graph object (with nodes and vertices), I've updated throughout the paper the word ``graph" into ``spectrogram image", or ``image stripe", depending on which part of the image the \textit{graph} was referring to. So please follow this if you are adding any mention of graphs.}\kl{Noted.}

\subsubsection{Vision Transformer}\label{subsec:visiontransformer}
In the next stage, the ViT-num-spec employs a vision transformer architecture that integrates a MLP head for the purpose of forecasting time series. The input images are segmented into non-overlapping patches of uniform size, effectively partitioning the horizontal time axis into discrete intervals corresponding to each image patch. These patches undergo linear projection to be transformed into tokens, augmented with standard 1D positional embeddings to maintain temporal ordering. The encoder is tasked with converting these patches into latent representations or feature vectors. For our implementation, we configure the input image dimensions to 128×128 pixels, with each patch sized at 16×16 pixels. The time series data from price movements is formatted to fit a 16×128 top row, while the spectrogram occupies a 112×128 space below it, ensuring compatibility with the patch size for optimal processing.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth, height=11em]{figs/workflow.png}
    \caption{
    %Overview of the proposed `data to predictions' workflow with ViT-num-spec \cite{zeng2023from} as the MM-TSFM. The path highlighted with black arrows denotes the path in which no perturbations are applied, blue arrows denote semantic perturbations (SP), green arrows denote composite perturbations (CP), and red arrows denote input-specific perturbations (IP). The generated predictions will be used for rating in the next step.
    Overview of our proposed `data to predictions' workflow with ViT-num-spec \cite{zeng2023from} showing different perturbation pathways: black arrows for no perturbations, blue for semantic (SP), green for composite (CP), and red for input-specific (IP). Predictions from these pathways are rated in the next step.
    % \sunandita{made the caption shorter. please check.}
    }
	\label{fig:system-workflow}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth, height=12em]{figs/perturbations.png}
    %scale = 0.95
    \caption{Unperturbed image and its perturbed variations, along with a corresponding difference image that highlights (in red) the portion that is modified after perturbation. In (f,g), the single pixel change is highlighted with a white circle around it.
    % (a) P0, no perturbation; (b, c) P1, a zero added to each row of the tabular time-series data; (d, e) P2, one value in each row of tabular time-series data is halved. (f, g) P3, the central pixel was altered to black (highlighted with a white circle); (h, i) P4, image saturation increased by 10 units; (j, k) CP, composite perturbation where the original time-series intensities are replaced with sentiment intensities from a CLIP-based sentiment analyzer.
    % \sunandita{The names are pretty self explanatory. Can remove the details about each perturbation and refer to the section in the paper.}
    }
    \label{fig:perturbations}
    \end{figure*}
    % \vspace{-0.6cm}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.35\textwidth, height=13em]{figs/rating-workflow.png}
    \caption{Our proposed 'predictions to ratings' workflow that performs statistical and causal analysis to compute raw scores and assign final ratings to the test systems.}
	\label{fig:rating-workflow}
\end{figure}

\subsection{Perturbations}
\label{sec:perturbations}
We assess the robustness of the models described in \nameref{sec:models} section by subjecting the input data to different perturbations across three different settings:
\subsubsection{Semantic Perturbation (SP)}
Semantic perturbations are alterations made to data that change its meaning while preserving the overall context.
% These perturbations are meaningful within the domain to which they belong. 
For example, in time-series forecasting, a stock's value might change drastically due to errors in data entry, or it might fluctuate due to some market-specific catalyst that affects certain companies. Under SP, we consider two perturbations:


\noindent {\bf 1. Drop-to-zero (P1):} It is inspired by 
% the stuck-at-zero fault in digital circuits due to which a signal will be permanently stuck at a logic level zero \cite{mei1974bridging} and 
the common data entry errors \cite{ley2019analysis}. We set every $80^{th}$ value in the original stock price data collected from the source to zero. Once converted into a sliding window format with 80 timesteps per row, this approach ensures that each row contains at least one zero.


\noindent {\bf 2. Value halved (P2):} In this setting, we reduce every $80^{th}$ number in the original stock price data to half of its value. This perturbation simulates periodic adjustments, possibly reflecting events like stock splits or dividend payments. 


\subsubsection{Input-specific Perturbation (IP)}
Input-specific perturbations are alterations specific to the mode - features and context of the data being used. In time-series forecasting, altering some pixels (e.g., changing their color) in a time-frequency spectrogram image is one example. Under IP, we consider two different perturbations:


\noindent {\bf 1. Single pixel change (P3):} In \cite{su2019one}, the authors modified a single pixel in each of the test images. With this approach, they fooled three types of DNNs trained on the CIFAR dataset. 
% They used differential evolution to find the most effective pixel modification to fool the DNN. 
In our work, we alter the center pixel of each multi-modal input to black based on the intuition that 
% . We demonstrate that even this 
small and consistent change to the images can significantly alter the models' prediction.


\noindent {\bf 2. Saturation change (P4):} In \cite{zhu2023imperceptible}, the authors showed that the adversarial perturbations in the S-channel (or saturation channel) of an image in HSV (Hue Saturation Value) form ensures a high success rate for attacks compared to other channels. 
% They generated perturbations on the S-channel in an iterative manner until the attack was successful. 
% Inspired from \cite{zhu2023imperceptible}, 
In our work, we increase the saturation of the multi-modal input ten-fold 
based on the intuition that a subtle change can affect the models' predictions.

\subsubsection{Composite Perturbation (CP or P5)}
We consider a composite case in which the MM-TSFM is combined with another AI system. This is because it is well known in finance that stock prediction can be influenced by market sentiment \cite{senti-bias-finance} and we want to explore such a realistic case. In \cite{kausik2023the}, the authors considered a composite case in which the input text is round-trip translated (translation from one language to the same through another intermediate language) and passed to a sentiment analysis system (SAS). Then they used the rating method to assess the bias in the system. In our work, we assess the sentiment of each time series by passing the corresponding time-series plot to a zero-shot CLIP-based \cite{radford2021learning, bondielli2021leveraging} sentiment analysis system ($S_c$) %(described in \ref{sec:models})
which outputs the sentiment intensity values (negative (-1), neutral (0), or positive (1)). These labels are scaled to values in the range [0, 255] and represented as sentiment intensity stripe and passed to MM-TSFM in place of the original time-series intensity stripe. This zero-shot CLIP-based $S_c$ for sentiment analysis may exhibit bias or may be inaccurate, the goal is to study the robustness of MM-TSFM in conjunction with such AI system.

\subsection{Workflow}
\label{sec:rating}

\subsubsection{From Data to Predictions:}


Figure \ref{fig:system-workflow} shows the overview of the proposed workflow with the ViT-num-spec model as the MM-TSFM. The paths highlighted in different colors correspond to different perturbations. The semantic perturbations (highlighted in blue), when applied to the numerical time-series data, are reflected in the corresponding spectrogram and the time-intensity images. The composite perturbation (highlighted in green), when applied, gets reflected in the corresponding time-series intensity image stripe. The spectrogram remains unperturbed. The input-specific perturbation (highlighted in red), directly affects both the spectrogram and the time intensities images. These perturbed/unperturbed input data points are fed to the MM-TSFM. The model processes the input (as described in \nameref{sec:models}) and predicts the next `d' timesteps (we set $d = 20$).

\subsubsection{From Predictions to Ratings:}
In \cite{kausik2024rating}, the authors introduced an approach to rate text-based sentiment analysis systems for bias. The rating algorithms we adapted from their paper are provided in Section 2 of the supplementary. We modify this approach to better suit our setting as it involves multi-modal data which is more complex than the textual data that was used in the original rating work. Also, our approaches involve multiple treatments (perturbations). Figure \ref{fig:rating-workflow} shows the overview of the proposed rating workflow. After preprocessing the data (optional), the first step is to check for sensitive attributes that may act as confounders. If they do not act as confounders, statistical methods to answer RQ1 from Section \nameref{sec:problem} would suffice. The metric used to assess the statistical bias is described in Section \ref{sec:metrics}. If they do act as confounders, causal analysis is necessary. We use two metrics: one to assess the impact of each perturbation and another to compute the confounding bias (to answer RQ2 and RQ3) respectively. These metrics are collectively referred to as raw scores (that form a partial order together) which aid in assigning the final ratings to the systems (that form a final order together). The range of final ratings depend on the value of rating level, L. The final ratings computed from our experiments are shown in Table \ref{tab:ratings-pie}.


==> AIES2024/sections/problem.tex <==
\section{Problem}
\label{sec:problem}
\subsection{Preliminaries}
\subsubsection{Stock Price Prediction:}
Let the time-series be represented by \{x$_{t-n+1}$, x$_{t-n+2}$, ...., x$_{t}$, x$_{t+1}$, ..., x$_{t+d}$\}, where each x$_{t-n+i}$ represents an adjusted closing stock price and $n$ and $d$ are  parameters. $n$ is called the sliding window size and $d$ is the number of future stock prices the model predicts.    
    In this sequence, let 
    X$_{t}$ $=$ \{x$_{t-n+1}$, x$_{t-n+2}$, ...., x$_{t}$\}, and let  $\hat{Y_{t}}$ $=$ \{x$_{t+1}$, 
    x$_{t+2}$, ...., x$_{t+d}$\}, where $\hat{Y_{t}}$ = f(X$_{t}$) i.e., based on the stock prices at previous $n$ timesteps, let the function $f$ represent an MM-TSFM that predicts the stock prices for the next `d' timesteps. Let $Y_{t}$ denote the true stock prices for the next `d' timesteps. Let $S$ be the set of time-series forecasting systems we want to assess. Let R$_{t}$ be the residual for the sliding window [t + 1, t + d] and is computed by ($\hat{Y_{t}}$ - $Y_{t}$) at each timestep. 

As the objective of our rating method is to consider the worst possible case (in this case, residual) to communicate the worst possible behavior of the model to the end-user, let us consider the MAX(R$_{t}$). Let it be denoted by $R^{max}_{t}$. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.25\textwidth]{figs/Causal_General.png}
	\caption{Causal diagram $\mathcal{M}$ for MM-TSFM. The validity of link `1' depends on the data distribution, while the validity of links `2' and `3' (with `?') are tested in our experiments.}
	\label{fig:causal-model}
\end{figure}

\vspace{-1em}
\subsubsection{Causal Analysis:}
Let the causal model that represents the system be denoted by \( \mathcal{M} \) - it is diagrammatically represented in  Figure \ref{fig:causal-model}. The arrowhead direction shows the causal direction from cause to effect. In Figure \ref{fig:causal-model}, if \emph{Sensitive Attribute} ($Z$) acts as a common cause for both \emph{Perturbation} ($P$) and \emph{Residual} ($R^{max}_{t}$), that would add a spurious correlation between the $P$ and the $R^{max}_{t}$. This is also called the confounding effect and \emph{Sensitive Attribute} is considered the confounder in this case. In the presence of a confounder, the path from \emph{Perturbation} to \emph{Residual} through the confounder is called a backdoor path and such a path is considered undesirable. Several backdoor adjustment techniques were used in the literature to remove the confounding effect \cite{xu2022neural, fang2024backdoor, liu2021preferences}. The deconfounded distribution (after backdoor adjustment) is represented by: $(R^{max}_{t} | do(P))$. The `do()' in causal inference denotes an intervention used to measure the causal effect of $P$ on the outcome. The solid red arrows in Figure \ref{fig:causal-model} denote the causal links whose validity and strength will be tested through our experiments. The dotted red arrow denotes the causal link that may or may not be present based on the distribution $(Perturbation | Sensitive Attribute)$ across different values of the \textit{Sensitive Attribute} i.e. if any perturbation that is applied depends on the values of $Z$. 

\subsection{Problem Formulation}
We aim to answer the following questions through our causal analysis when different perturbations denoted by $P$ = \{0, 1, 2, ..\} (or simply $P0, P1,...., P5$) are applied to the input given to the set of time-series forecasting systems $S$:


\noindent{\bf RQ1: Does $Z$ affect $R^{max}_{t}$ of $S$, even though $Z$ has no effect on $P$?}
    %\sunandita{to discuss: how can a protected feature Z have an impact on a perturbation P we are doing? Do you mean effect on the outcome of doing the perturbation?} \kl{I framed the the question in causal terms? The literal meaning is: "if the applied perturbation does not depend on the value of the confounder (company or the industry)".}

\noindent That is, if the applied perturbations do not depend on the value of the sensitive attribute, would the sensitive attribute still affect the system outcome leading to a statistical bias? In this case, causal analysis is not required to answer the question as there is no confounding effect. 
    % Mathematically, are the distributions $(R^{max}_{t} | Z)$ statistically different for different values of $Z$? If yes, this implies that $S$ exhibits \textbf{statistical bias}.

\noindent {\bf RQ2: Does $Z$ affect the relationship between $P$ and $R^{max}_{t}$ of $S$ when $Z$ has an effect on $P$?}

\noindent That is, if the applied perturbations depend on the value of the sensitive attribute, would the sensitive attribute add a spurious (false) correlation between the perturbation and the outcome of a system leading to confounding bias? 
    % still affect the system outcome leading to a statistical bias? Causal analysis is not required to answer this question as there is no confounding effect. 
    % Mathematically, is $(R^{max}_{t} | do(P))$ = $(R^{max}_{t} | P)$? i.e., are observational and interventional distributions equal? If the answer is no, it implies that $S$ exhibits \textbf{Confounding bias}.

\noindent {\bf RQ3: Does $P$ affect $R^{max}_{t}$ of $S$ when $Z$ has an effect on $P$?}

    % Mathematically, is $|E(R^{max}_{t} = j| do(P = i)) - E(R^{max}_{t} = j| do(P = 0)|$ = 0? i.e., the expectation of interventional distributions of $R^{max}_{t}$ for perturbed and control (or unperturbed) groups the same? If yes, this implies that the perturbation does not have any effect on $R^{max}_t$ of $S$. 
\noindent That is, if the applied perturbations depend on the value of the sensitive attribute, what is the impact of the perturbation on the outcome of a system?

\noindent {\bf RQ4: Does $P$ affect $\hat{Y_{t}}$ of $S$ in the presence of $P$?}

\noindent That is, do the perturbations affect the performance of the systems in terms of accuracy? Causal analysis is not required to answer this question as we only need to compute appropriate accuracy metrics to assess how robust a system is against different perturbations.
    % $S$ is against $P$ in terms of accuracy. Mathematically, is $\hat{Y_{t}}$ different from $Y_{t}$ in presence of no perturbation (P0) and different perturbations (P1 through P5).




==> Common/sections/approach.tex <==
\section{Approach}
\subsection{Datasets}
\begin{enumerate}
    \item EmoAtCap dataset
    \item Emoji Sentiment
    % \item CMU-MOSI with gender annotation for audio files.
    % \item RAVDESS dataset
\end{enumerate}

\subsection{Models}
\subsubsection{I-SAS}
\begin{enumerate}
    \item Deep-Emotion or Transfer Learning using MobileNetV2
    \item DeepFace
    \item CLIP
    \item BLIP
\end{enumerate}
\subsubsection{MM-SAS}
\begin{enumerate}
    \item Bi-Bimodal Modality Fusion for Correlation-Controlled Multimodal Sentiment Analysis.
    \item MISA: Modality-Invariant and -Specific Representations for Multimodal Sentiment Analysis.
\end{enumerate}




\subsubsection{CLIP Model: Zero-shot Classification}

\subsubsection{Deep-Emotion Model}
The deep Emotion model was proposed in \cite{deep-emotion}.

==> Common/sections/case-study.tex <==
\section{Case Study}
\subsection{Case Study A: Sentiment Analysis}
\subsection{Case Study B: Car Score Prediction}


==> Common/sections/discussion.tex <==
\section{Discussion}
% If the person is faking their emotion, bio-signals help us identify their true emotions. Each of the emotions can be further classified into the intensity of emotions (regression task).

Let S be a pre-trained AI system that was trained on the task of image-text alignment. Given a set of images and captions, the image-text alignment task targets to close the distance of paired image-text and enlarge that of the unpaired ones \cite{wei2022icar}. For example, the CLIP \cite{radford2021learning} model learns a multi-modal embedding space by jointly training image and text encoders to maximize the cosine similarity between the image and text embeddings of N real pairs in a batch while minimizing the cosine similarity of the embeddings of the $N^2 - N$ incorrect pairings. 

==> Common/sections/introduction.tex <==
\section{Introduction}
Legend:
\begin{itemize}
    \item I-SAS: Image-based SAS
    \item T-SAS: Text-based SAS
    \item MM-SAS: Multi-modal SAS that gives a combined prediction based on multiple modalities. In this paper, we only consider images and text.
\end{itemize}


Necessary ingredients:
\begin{enumerate}
    \item Project Scope
    \item Contributions
    \item Data
    \item Systems
    \item Experimental Design
    \item Metrics and Evaluation
\end{enumerate}

We answer the following research questions through this work:
\begin{enumerate}
    \item Does the I-SAS sentiment prediction change based on transformations like changes in lighting, background, orientation, etc. in the image?
    \item Does the I-SAS sentiment prediction change based on the gender of the subject(s) in the image?
\end{enumerate}

==> Common/sections/problem.tex <==
\section{Problem}
\subsection{Notation}
% Let S be a pre-trained AI system that was trained on the task of image-text alignment. Given a set of images and captions, the image-text alignment task targets to close the distance of paired image-text and enlarge that of the unpaired ones \cite{wei2022icar}. For example, the CLIP \cite{radford2021learning} model learns a multi-modal embedding space by jointly training image and text encoders to maximize the cosine similarity between the image and text embeddings of N real pairs in a batch while minimizing the cosine similarity of the embeddings of the $N_2 - N$ incorrect pairings. 
Let a multi-modal classifier that predicts the class of the provided input be denoted by $S_C$. Let I be the set of input images, T be the set of corresponding textual descriptions, and C be the additional class information. A sentence like "This is an image with positive sentiment." can be a part of set C. Let $I_o$ and $T_o$ denote blank image and blank text respectively. Let the true class (ground truth) of the input be Y. Let the input features be denoted by $F$ and it constitutes the image, class information, and textual features which are denoted by $F_I$, $F_C$, and $F_T$ respectively. These features can again be classified into the following categories:
\begin{enumerate}
    \item Desirable Features (D): The features that ideally should be the only features responsible for the prediction made by S. Let the desirable features of image, class information, and text be denoted by $D_I$, $D_C$, and $D_T$ respectively.
    \item Protected Features (Z): The features that should not affect the outcome of $S_C$. Let the protected features of the image, class information, and text be denoted by $Z_I$, $Z_C$, and $Z_T$ respectively.
\end{enumerate}

\subsection{Task Formulation}
Let $f$ be a function that maps the input features to a class i.e., $f$: $F$ $\rightarrow$  $\hat{Y}$. In simpler words, when (I, T, C) is provided as an input to $S_C$, it outputs the C with the maximum confidence. This will be the final output, $\hat{Y}$.


\subsection{Problem Formulation}
In this paper, we evaluate $S_C$ for bias through causal analysis. If $Z$ affects $\hat{Y}$, it can be called as statistical bias. If $Z$ is acting as a confounder that adds a spurious correlation between the input and the output, then it can be called as confounding bias. If there is a difference between the observational and experimental distributions of ($\hat{Y}$ $|$ $X$), then the system is said to exhibit confounding bias. $\psi$ denotes the DIE\% or WRS scores computed based on whether $Z$ acts as a confounder or not. $\psi$ can be called as the raw score that can be used to rate $S_C$.
We test different hypotheses and consider different compositional cases by combining different modalities. 

\begin{enumerate}
    \item Unimodal Analysis: 
    \begin{itemize}
        \item Image: (I, $T_o$, C) is given as input to S. $T_o$ indicates that the text is $\emptyset$. So, we provide an empty string in its place, along with I and C. Let the raw score for this system be $\psi_I$
        \item Text: ($I_o$, T, C) is given as input to S. $I_o$ indicates that the image is $\emptyset$. So, we provide a blackened image in its place, along with T and C. Let the raw score for this system be $\psi_T$
    \end{itemize}
    \item Multi-modal Analysis: (I, T, C) is given as input to S. Let the raw score for this system be $\psi_{IT}$.
    \end{enumerate}

    \subsubsection{Compositional Problem:} 
    Is there a relation between the individual raw scores from the unimodal analysis and the combined raw score from the multimodal analysis? This problem can be formally defined as: 
    
    $h(\psi_{m1}, \psi_{m2}, ..., \psi_{mk}) \leq \psi_{m_{1}m_{2}...m_{k}} \leq g(\psi_{m1}, \psi_{m2}, ..., \psi_{mk})$

    where $(m_1, m2, ...m_k) \in M$ denote the set of different modalities. I and T are the modalities we consider in this paper. 

% \subsection{Experimental Design}





==> Common/sections/related_work.tex <==
\section{Related Work}
\subsection{Multimodal Classification Systems}
\subsection{Bias in AI Systems}
\subsection{Evaluating Bias in Multimodal AI Systems}


\subsection{Evaluating AI Systems for Bias using Causal Analysis}
Some of the previous works used causality to make the object recognition systems more robust from confounding factors like background and viewpoints. In \cite{mao2021generative}, the authors make generative models to intervene on features caused by confounding factors like background, viewpoint, and scene contexts. This enables robust generalization. In \cite{mao2022causal}, the authors show that the association between image and label is not generalizable (or not transportable, in causal language). In \cite{wang2021causal}, the authors show that confounders like the background in the image might trick the attention module into capturing spurious correlations that benefit the model when training and test data are IID but harm the prediction when tested on OOD images. To address this problem, besides using standard attention that attends to the desired causal features like foreground, the proposed model uses complementary attention that captures the background. These two disentangled attentions are optimized in an adversarial minimax manner, mitigating the confounding bias in an unsupervised way.   


\subsection{Rating of AI Systems for Bias}

\subsection{Composite Rating}
In \cite{tran2019bayesian}, the authors introduce BayesianLayers, a module designed for capturing neural network uncertainty. These layers capture these uncertainties overweights, pre-activation layers, and activation units. Instead of using deterministic functions as layers, they enable distribution over functions and introduce uncertainty-aware models as a composition of layers. They swap the layers to propagate uncertainty from the input to the output. They do not compute the composition of two neural networks but only consider the composition of layers in the context of uncertainty propagation through a single neural network. In \cite{jirouvsek2013brief}, the author discusses an approach to multidimensional probability distribution representation based on composition. This is an alternative approach to Bayesian networks. The Composition is defined as inverse marginalization. It combines two distributions into a single distribution by multiplying two marginal distributions and marginalizing the result over the variables present in both distributions. In \cite{d2020survey}, the authors investigate different types of linear and non-linear composition operators in Lipschitz and Baire function spaces. However, the function spaces discussed do not apply to our setting.

==> Common/sections/rough.tex <==
% \section{Problem}
Some resources: 
1. (Data) Downloaded annotations for COCO dataset (on Mac): \url{https://princetonvisualai.github.io/imagecaptioning-bias/}. 




